Discourse-level Relation Extraction via Graph Pooling

The ability to capture complex linguistic structures and long-term dependencies among words in the passage is essential for discourse-level relation extraction (DRE) tasks. Graph neural networks (GNNs), one of the methods to encode dependency graphs, have been shown effective in prior works for DRE. However, relatively little attention has been paid to receptive fields of GNNs, which can be crucial for cases with extremely long text that requires discourse understanding. In this work, we leverage the idea of graph pooling and propose to use pooling-unpooling framework on DRE tasks. The pooling branch reduces the graph size and enables the GNNs to obtain larger receptive fields within fewer layers; the unpooling branch restores the pooled graph to its original resolution so that representations for entity mention can be extracted. We propose Clause Matching (CM), a novel linguistically inspired graph pooling method for NLP tasks. Experiments on two DRE datasets demonstrate that our models significantly improve over baselines when modeling long-term dependencies is required, which shows the effectiveness of the pooling-unpooling framework and our CM pooling method.

==> sections/0_Introduction.tex <==
\section{Introduction}
\label{Introduction}
%\hl{RE is important for automatic knowledge base construction; and result re community start to look at document-level RE}
Relation extraction, the task to extract the relation between entities in the text, is an important intermediate step for automatic knowledge base construction \cite{DBLP:conf/doceng/Al-ZaidyG17, dong2014knowledge}. %, which benefits many downstream applications such as question answering~\cite{xu-etal-2016-question}, knowledge base population, and coreference resolution~\cite{luan2018multi}. 
While earlier works in relation extraction focus relations within a single sentence \cite{DBLP:conf/emnlp/XuFHZ15,DBLP:conf/acl/MiwaB16}, recent works place more emphasis on identifying the relation between entities that appear at discourse level \cite{DBLP:conf/naacl/JiaWP19,DBLP:conf/aaai/XuCZ21}, which is more practical yet challenging to models. Most notably, models need to consider larger amount of information and capture the complex interaction between entities and their mentions for each relation\footnote{An entity can be mentioned multiple times with different surface form in the context.}.
%For example, in Fig.~\ref{intro_fig}, the relation between \textit{Cystitis} and \textit{Adrimycin} can only be understood by considering the whole paragraph.

%\hl{recent research on DRE mostly follow a pipeline that xxxx. and propose variations to capture interaction between mentions and entities given an extracted mention representations. However, this kind of pipeline isolate the context reasoning stage and structure reasoning stage .. stuctured guidance in the first place. Thus, how to learn a better mention representation that can xxxx is important. Need figure}
Many previous works that study discourse-level relation extraction (DRE) address the task following a paradigm that first uses a general-purpose encoder, such as BERT \cite{BERT}, to obtain the representations of entity mentions, and then construct entity embeddings from the mention representations by applying graph-based models, which capture the interaction between different mentions, entities, and their structures \cite{DBLP:conf/emnlp/ChristopoulouMA19, DBLP:conf/emnlp/ZengXCL20, DBLP:conf/emnlp/WangHCS20}. Although obtaining great success, these kinds of approaches isolate the context reasoning stage and entity structure reasoning stage, which means the context information cannot be learn together with structural information.
To address the issue, \citet{DBLP:conf/aaai/XuWLZM21} propose SSAN that incorporates structural dependencies between entity mentions within the encoding stage. Even without the additional graph-based models that calibrate final entity embeddings from their corresponding mention representation, their approach can obtain competitive results on DRE tasks by simply aggregating mention representations with average pooling to form entity embeddings.
%\hl{With minimal design to aggregate entity information from the better mention representations, their approach can obtain competitive results on document level RE tasks.}

Following the success of SSAN, we aim at learning mention representations that can capture structural dependencies together with context for DRE tasks. 
SSAN only considers co-occurrence and coreference structure between entity mention tokens, while we tend to add more structural information to learn a richer mention representation. 
For example, incorporating dependency tree structures to capture syntactic clues have been shown effective in sentence-level relation extraction \cite{DBLP:conf/emnlp/Zhang0M18}.
These dependencies can usually be depicted as graphs with nodes representing tokens and edges representing the dependencies. In general, models that can encode graphs, such as Graph Convolutional Networks (GCN)~\cite{DBLP:conf/iclr/KipfW17}, Graph Attention Networks~\cite{DBLP:journals/corr/abs-1710-10903}, or even networks that modify Transformers (like SSAN), can all help model the structure. However, when the input text scale comes to discourse level, it requires additional efforts, such as stacking a deep network to aggregate information between nodes that are with long distance.

%\hl{In this work, we propose to use graph pooling unpooling framework to faciliate the mention representation learning in DRE. }
To address this issue and facilitate the mention representation learning in DRE, in this work, we leverage the idea of \textit{graph pooling} and propose to use a pooling-unpooling framework (as depicted in Figure~\ref{Architecture}). In the pooling branch, we use \textit{graph pooling} to convert the input graph to a series of more compact hypergraphs by merging structurally similar or related nodes. The graph node representation learning on the hypergraph thus aggregates a larger neighborhood of features compared to the learning on the original graph. Such pooling technique alleviates the pain of capturing long dependencies, while keeping the structural information between nodes. Then, we introduce the unpooling layers to restore global information in hypergraphs back to the original graph so that embeddings for each entity mention can be extracted.


We use GCN, one of the most commonly-used methods to encode graphs, to instantiate our proposed pooling-unpooling framework. Additionally, we explore two graph pooling strategies -- Hybrid Matching and Clause Matching to justify our method's generalizability. Hybrid Matching (HM)~\cite{DBLP:conf/icwsm/LiangG021} merges nodes based on the structural similarity and get success in learning large-scale graph. However, HM ignores the edge type information when merges nodes, which could be helpful to group nodes. For example, nodes linked with \textit{``nmod''} dependency edge can often be merged when considering its linguistic meaning in text\footnote{The definition of nmod in Universal Dependencies \cite{DBLP:conf/lrec/NivreMGHMPSTZ20} is: \textit{``The nmod relation is used for nominal dependents of another noun or noun phrase and functionally corresponds to an attribute, or genitive complement.''}}. Thus, we propose Clause Matching (CM) to leverage the type information within dependent arcs to merge nodes. 
%Comparing to HM, which is a general graph pooling algorithm that merges nodes by considering the overall graph structure, CM is designed from the linguistic perspective and specifically focuses on dependent relations between nodes.
Despite the differences, our proposed method with either pooling method achieves substantial improvements over baselines on two DRE datasets -- CDR~\cite{CDR} and cross-sentence $n$-ary~\cite{nary}.

To sum up, our contributions are: 
(1) We introduce the idea of using pooling-unpooling framework to learn structural dependencies for entity mention representations in DRE tasks. The framework is agnostic to the graph pooling method and to the model that encode graphs.
(2) We introduce a new graph pooling method -- Clause Matching (CM), which merges tokens based on their dependency relations. CM can largely reduce the graph size while keeping the semantic structure of the input. 
(3) We carry out comprehensive experiments and analysis on two DRE datasets to understand the proposed framework. With detailed comparisons to the baselines, we verify the pooling-unpooling framework's effectiveness, especially in cases needing consideration on long dependencies.
%(3) We study our framework and CM on two DRE datasets. With detailed comparison to the baselines, we verify the pooling-unpooling framework's effectiveness. 
%(3) We carry out a comprehensive analysis to understand the proposed framework, including an analysis that studies the \textit{entity distance} in graph, which shows that the pooling-unpooling mechanism is effective for predicting relations among entities with long distances.

\iffalse
\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{images/intro_fig_crop.pdf}
\caption{An example of document-level relations from the CDR dataset. The oval represents chemical \textcolor{red}{\textbf{\textit{Adriamycin}}}, and rectangles represent two diseases: \textcolor{myblue_2}{\textbf{\textit{Bladder Carcinoma}}} and \textcolor{mygreen}{\textbf{\textit{Cystitis}}}. Reading the whole passage over six sentences is essential to the understanding about the relation between \textcolor{red}{\textbf{\textit{Adriamycin}}} and \textcolor{mygreen}{\textbf{\textit{Cystitis}}}. }
% It is necessary to read the whole passage over six sentences to understand the relation between \textcolor{red}{\textbf{\textit{Adriamycin}}} and \textcolor{mygreen}{\textbf{\textit{Cystitis}}}. }
\label{intro_fig}
\vspace{-1.5em}l;
\end{figure}
\fi

\begin{figure*}[t!]
\centering
    \includegraphics[width = 0.85\linewidth]{images/models/mirror_GCN.pdf}
    \vspace{-0.5em}
	\caption{Our proposed pooling-unpooling framework: Input words are first encoded into vectors and then fed into pooling-unpooling layers to learn the structural dependencies within the input tokens. GNN block can be any model that encode graphs and update node embeddings. Pooling layers merges nodes in the original graph into supernodes, forming smaller size graphs. Unpooling layers map the information from the coarser graph back to finer-grained graph. 
	%This pooling-unpooling design helps the model aggregate structural information with different scales, which alleviate the model's pain on capturing long dependencies in the original graph. 
	In the figure, $G_i$ represents hypergraphs at the $i$-th level. $H_i^{in}$ and $U_i^{in}$ denote the converted embeddings after the pooling and unpooling layers in $i$-th hypergraph. Both of them can be calculated using the matching matrix $M_{l,l+1}$. We use $H_i^{out}$ and $U_i^{out}$ to denote the refined representations after GNN blocks.}
	\label{Architecture}
	\vspace{-1.05em}
\end{figure*}



==> sections/3_3_GCN.tex <==
\subsection{Graph Convolutional Network}
\label{ssec:gcn}
Given the hypergraphs that we have generated through graph pooling, graph convolution networks (GCN)~\cite{kipf2016semi} is executed to update node embeddings on the hypergraphs. %GCN~\cite{kipf2016semi} is an extension of Convolutional Neural Network~\cite{lecun1998gradient} for non-euclidean graphs. 
%The GCN block in our model is a stacked GCN with $S$ layers ($S\in \mathbb{Z}^+$),
%where $S$ is a hyperparameter. 
We stack $S$ layers ($S\in \mathbb{Z}^+$) of GCN for a GCN block, and we do not adopt complex techniques, such as incorporating directionality or edge-wise gates~\cite{bastings2017graph,marcheggiani2017encoding} for simplicity.
% we do not adopt the techniques~\violets{what are those techniques for? can we give more details?} mentioned in \cite{bastings2017graph,marcheggiani2017encoding}.

With the adjacency matrix $A$ we introduced before,
%Given a graph $G$ with $n$ nodes, we represent the input graph with a $n\times n$ adjacency matrix $A$ with each entry $A_{ij}$ indicating an edge links from node $i$ to $j$.
the operation of the GCN block is:
\begin{equation}
\small
h_i^{l} = RELU(\sum_{j=1}^{N}A^l_{ij}W^{l}h_j^{l-1} + b^l), \label{eq:2}
\end{equation}
where $h_i^{l}$ is the representation of node $i$ in the $l$-th graph, and $W^{l}$ and $b^l$ are the corresponding weight and bias term.
% is the linear weight, and $b^l$ is a bias term in $l$-th layer. 
% In our cases, the adjacency matrices $A$ are different for different level of GCN block due to pooling layers and 
% We add self-loop to our adjacency matrices $A$: $\widetilde{A}=A+I$ ($I$ is the identity matrix) to emphasize the information residing in node itself. 
We define the output embedding $H^{out}_{l}$ of $G_{l}$ as $H^{out}_{l} = f_{GCN}(H^{in}_{l})$, 
% \begin{equation}
% \small
% H^{out}_{l} = f_{GCN}(H^{in}_{l})
% \label{Eq_unpooling}
% \end{equation}
where $f_{GCN}$ approximates the GCN block function.
% The GCN block in our proposed method is a stacked GCN with $S$ layers, where $S$ is a hyperparameter.
% %for aggregating features in graph node from the large distance and increase the representation learning ability \cite{kipf2016semi}. Also, 
% %In the spirit of simplifying 
% For the simplicity, 
% %our GCN backbone intends to highlight the advantages of our proposed method, 
% we do not adopt complex techniques in our GCN block, such as incorporating directionality or the edge-wise gates~\cite{bastings2017graph,marcheggiani2017encoding}.
% % we do not adopt the techniques~\violets{what are those techniques for? can we give more details?} mentioned in \cite{bastings2017graph,marcheggiani2017encoding}.



==> sections/6_Ablation_studies.tex <==
\begin{table}[t!]
\renewcommand{\tabcolsep}{1mm}
\centering
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{@{ }l@{ }|ll|ll|l@{ }}\toprule
\multirow{3}{*}{\textbf{Model}}   & \multicolumn{4}{c|}{\textbf{$n$-ary}}                & \multirow{3}{*}{\textbf{CDR}} \\ \cline{2-5}
                         & \multicolumn{2}{c|}{\small{Detection}} & \multicolumn{2}{c|}{\small{Classification}} &                           \\ \cline{2-5}
                         & \small{Ter.}        & \small{Bin.}       & \small{Ter.}        & \small{Bin.}        &                           \\ \hline
MrGCN(CM)            & 83.3$^{*}$       & \textbf{81.5}      & 77.4$^{**}$       & 76.0        & \textbf{65.6}$^{*}$                   \\
MrGCN(HM)            & \textbf{83.6}$^{*}$        & 81.4     & \textbf{78.3}$^{*}$        & \textbf{76.5}       & 64.7$^{*}$                \\
MrGCN-pool				   & 82.2	 & 81.2       & 76.8         & 76.2       & 62.7
\\
MrGCN(CM)-RNN                 & \textit{82.5}         & \textit{80.8}$^{*}$       & 75.4$^{*}$         & 73.4$^{*}$         & \textit{63.1}$^{*}$   \\
MrGCN(HM)-RNN                 & 82.2         & \textit{80.8}$^{*}$        & \textit{76.2}$^{*}$       & \textit{75.1}$^{*}$       & 61.9$^{*}$              
\\
MrGCN-pool-RNN      & 82.0        & 80.1       & 73.8        & 70.0        & 60.2                     \\
MrGCN-pool-RNN-Att. & 77.4        & 79.1       & 70.3        & 71.2    & N/A     \\ 
\bottomrule
\end{tabular}}
\caption{
Ablation studies. We report average accuracy for $n$-ary and F1 for CDR dataset. Ter. and Bin. 
stand for ternary and binary relation, respectively. 
No multi-head attention (Att.) component in models in the entity-centric dataset (e.g. CDR), so the setting in the last row is N/A. * and ** indicates the model outperforms its corresponding model without pooling with p-value $<$ 0.01 and $<$ 0.05 per McNemar's test, respectively. \textbf{Bold} and \textit{italic} indicate the best in each task and without RNN, respectively. 
}    
\label{tab:ablation_nary}
\end{table}
\section{Analysis and Discussion} %\violet{I will add several sentences to summarize the GOAL of the analysis. E.g., say we observed in the overall trends that MrGCN is especially good at handling long-term dependencies and complex cases. We want to conduct analysis to verify this hypothesis. (similarly for the ablation study, summarize why you want to do it.}
% In Sec.~\ref{results}, we have demonstrated the superiority of MrGCN over baselines. 
In this section, we investigate how MrGCN benefits from its components and verify the hypothesis that \textit{Graph Pooling} is especially efficient for capturing long-term dependencies. 
% Yet, we have not shown the origin of the advantage. Hence, we plan to investigate the merits of different components in MrGCN (Sec.~\ref{ablation_study}).
%Especially, in Sec.~\ref{perf_len},~\ref{perf_ent}, we verify our hypothesis on that the idea of \textit{Graph Pooling} can help model capture long-term dependencies more efficiently and effectively. The results provide supporting evidences that MrGCN performs well in scenarios where long-term dependencies are required.
% MrGCN performs excellently in terms of handling cases with long-term dependency, 
% Secondly, we adapt the idea of \textit{Graph Pooling} in order to make models able to capture long-term dependencies more efficiently and effectively. 
% We want to conduct studies to verify the hypothesis that MrGCN is especially good at handling cases with long-term dependency (Sec.~\ref{perf_len},~\ref{perf_ent},~\ref{cdr_instance_type}).
%We use our best approach, i.e, MrGCN(HM), to conduct these analyses.
%We conduct detailed analyses on our best approach, i.e, MrGCN(HM).
%MrGCN model with Hybrid Matching method.
%, since it shows better performance on the $n$-ary dataset. Further, 

Noted that Entity Anonymity setup is more principled under the distant supervision setting,
%like the $n$-ary dataset, 
so in this section, the results on the $n$-ary dataset are obtained under the Entity Anonymity setup.
%all the anaylsis  are done under Entity Anonymity setting if the result is shown on the $n$-ary dataset.
\subsection{Ablation Studies}
\label{ablation_study}
We present ablation studies in Table~\ref{tab:ablation_nary}. 
For models \textit{without RNN} (Rows 4-6), by comparing the models with and without pooling, we observe that graph pooling indeed significantly improved the performances on both datasets. %In the $n$-ary dataset, the improvements are at least 0.7 accuracy increase in 3 out of 4 sub-tasks. As for the CDR dataset, pooling brings at least 1.7 F1 scores boost. 
Likewise, ablating pooling from full MrGCN models (Rows 1-3) leads to significant performances decrease, especially on the CDR dataset. % in which the difference is 2.0 F1 scores
Also, the benefits brought by the pooling mechanism is more significant on the CDR dataset and $n$-ary dataset's ternary cases, where we anticipate longer distances between entities.
% the more complex ternary cases for $n$-ary. 
%We hypothesize the reason being that instances in CDR dataset and n-ary ternary cases have the longer distance, 
%than binary case in $n$-ary. 
%which can further highlight the importance of the pooling-unpooling mechanism to handle complex cases.
%
BiLSTM (RNN) layers are useful for both datasets, and the attention mechanism is also efficient. Importantly, graph pooling is shown to be complimentary to these mechanisms as it brings performance gains on top of these sophisticated techniques.   %, where removal of BiLSTM causes the performance drop.
% and its contribution is independent with other components.
% our pooling-unpooling architecture, 
% As we know, GCN is relatively incapable of carrying sequential information in the context, which is crucial to learn the semantics. Conversely, 
% %This raises a issue 
% % This observation also indicates that 
% BiLSTM's contextualized embeddings provide us a way to learn such sequential information. Using positional embedding~\cite{vaswani2017attention, gao2019learning} to provide original relative position information might be a potential alternative to BiLSTM, which we leave to the future work. 


\begin{figure*}[t]
\centering
    \includegraphics[width=\linewidth]{images/results/overall.pdf}
	\caption{Performance against input length and entity distance in graph.}
	\label{entity_distances}
\end{figure*}

\subsection{Performance against Input Length}
\label{perf_len}
We follow \citet{song2018n} to conduct analysis about 
%to study 
model performance against input length, which has been reported in Fig.~\ref{entity_distances}a. In CDR dataset, the performance differences between models with and without pooling gradually increase when the input sentences grow longer, especially when the text length is over 375 tokens (while the difference is not significant when the input sentence is less than 250 words). In $n$-ary dataset, the performance gap between models with and without pooling is significant when sentence length is between 75 to 100, yet the performances within shorter sentence length are similar.
%gradually increase when the input sentences grow longer. 
%the performance difference reaches 5.4 F1 scores when the text length is over 375 tokens, while the difference is not significant when the input sentence is less than 325 words.
Such observations demonstrates that the pooling-unpooling mechanism helps cases with longer context.

%In CDR dataset, the model notably without Bi-LSTM and pooling performs as good as \textit{MrGCN(HM)} in short instances, but its performance degrades severely when the input becomes lengthier. 
%Conversely, such performance decay is less significant in \textit{MrGCN(HM)},
%, which even performs better when the text length is over 300 tokens. 
%and our pooling method shows improvements when the text length is over 200 (\textit{MrGCN(HM)} vs. \textit{MrGCN(HM)-pooling}).

% \begin{figure}[t!]
% \centering
%     \includegraphics[width=0.9\linewidth, height=4.8cm]{images/results/n_ary_overall.png}
%     \includegraphics[width=0.9\linewidth, height=4.8cm]{images/results/CDR_result_overall.png}
% 	\caption{Performance against input length.}
% 	\label{sentence_length_n_ary}
% \end{figure}
% \begin{figure}[t!]
% \centering
%     \includegraphics[width=\linewidth]{images/results/Sen_len_result.png}
% 	\caption{Performance against input length.}
% 	\label{sentence_length_n_ary}
% \end{figure}
%A surprising observation 
Surprisingly, in CDR dataset,  MrGCN suffers from a performance drop on instances with sentence length between 325 and 375, which we hypothesize is due to our model selection strategy. Specifically, we select the model according to the overall performance, hence, the final model can possibly be biased.\footnote{The hypothesis also explains the phenomenon in Fig.~\ref{entity_distances}b} 
%Also, there are no significant performance differences under different sentence length for MrGCN without pooling. It is counterintuitive that we assume lengthier instances should be harder for models and usually have lower performances.
Yet, another notable observation is that there is no significant performance drop for MrGCN without pooling on lengthier input. %It is counter-intuitive since we usually think longer instances should be harder.
We hypothesize that sentence length is unnecessarily the best to measure %to judge an input instance requiring 
long-term dependencies between entities. %\footnote{We assume that instances require long-term dependencies are harder for models, and usually have lower performances.}. 
For instance, intuitively, although the inputs are long, the entities of interests are neighboring. 
% indicating that sentence length is  unnecessarily the best to measure long-term dependencies. 
%To better verify our claim that pooling-unpooling mechanism help model better learn the long-term dependency, %study the long-term dependency requirements, 
Hence, we propose \textit{entity distance} to study the model performance.
% to study the model performance against entity distances.
%Our hypothesis regarding such performance decrease is our way of the model selection.

% We offer two hypotheses regarding such performance decrease. First, it might be because of suboptimal merging operation between multiple entities in the document.  
%However, the overall trend in Figure \ref{sentence_length_n_ary} is clear: all models perform worse on the longer instances, but the performance downgrade is less significant for MrGCN.
\subsection{Performance against Entity Distance}
\label{perf_ent}
%To better estimate the dependencies between entities for making a relation prediction, we categorize each instance based on its entity distance in the document graph. 
We compute the \textit{entity distance} in the document graph for each instance.
% For each instance, we compute its entity distance based on the document graph. 
For mention-centric RE, we calculate the minimum distance between mentions in the graph, denoted as \textit{mention-pair distance}.\footnote{If mentions contain multiple tokens, we calculate average distances between each token pairs in the mention-pair.} Notably, in the ternary relation, the entity distance is the maximum value among three \textit{mention-pair distance}, since such an upper-bound estimation reflects the largest effort to capture the required dependencies.
%Then, we use the maximum distance among  In ternary relations, we use the maximum distance among the three mention pair distances to provide the upper-bound estimation. 
Similarly, for entity-centric RE, we first calculate the \textit{mention-pair distance}
%minimum distance 
between each targeted mention pairs that belongs to entity-pairs of interests.
% in the input graph, and 
Then, we take the maximum value over all \textit{mention-pair distance}.
% to be the entity distance. 

Fig.~\ref{entity_distances}b shows the result of MrGCN against different entity distance. We can observe that the performance for all models degrade significantly in CDR when the entity distance increases. In $n$-ary dataset, unlike the Fig.~\ref{entity_distances}a, the performances for model without pooling do not increase significantly as the entity distance grows. Such two tendencies indicate that \textit{entity distance} may reflect long-term dependencies between entities more precisely. 
%measures the difficulty of an instance. 
Also, with the help of graph pooling, MrGCN consistently outperforms MrGCN-pooling when \textit{entity distance}is larger than 4 in CDR, 3 in $n$-ary, which supports the effectiveness of using graph pooling for capturing long-term dependencies.





